ERNIE 3.0: Large-scale Knowledge Enhanced Pre-training for Language Understanding and Generation

Pre-trained models have achieved state-of-the-art results in various Natural Language Processing (NLP) tasks. Recent works such as T5 and GPT-3 have shown that scaling up pre-trained language models can improve their generalization abilities. Particularly, the GPT-3 model with 175 billion parameters shows its strong task-agnostic zero-shot/few-shot learning capabilities. Despite their success, these large-scale models are trained on plain texts without introducing knowledge such as linguistic knowledge and world knowledge. In addition, most large-scale models are trained in an auto-regressive way. As a result, this kind of traditional fine-tuning approach demonstrates relatively weak performance when solving downstream language understanding tasks. In order to solve the above problems, we propose a unified framework named ERNIE 3.0 for pre-training large-scale knowledge enhanced models. It fuses auto-regressive network and auto-encoding network, so that the trained model can be easily tailored for both natural language understanding and generation tasks with zero-shot learning, few-shot learning or fine-tuning. We trained the model with 10 billion parameters on a 4TB corpus consisting of plain texts and a large-scale knowledge graph. Empirical results show that the model outperforms the state-of-the-art models on 54 Chinese NLP tasks, and its English version achieves the first place on the SuperGLUE benchmark (July 3, 2021), surpassing the human performance by +0.8% (90.6% vs. 89.8%).

==> table_dataset_Chiness.tex <==
\begin{table*}[htb!]

  \tabcolsep 0.2in
	\begin{center}
    %\scriptsize
		\begin{tabular}{l|l|c|c|c|c|c}
		\hline \hline
			Corpus &Task& \#Train & \#Dev & \#Test   & \#Label &Metrics\\ \hline

      CMRC 2018     & MRC   & 10K     & 3.2K  & -  &  - & EM/F1 \\
      DRCD          & MRC   & 27K     & 3.5K  & 3.5K  &  - & EM/F1 \\
      DuReader      & MRC   & 271.5K  & 10K   & -   &  - & EM/F1 \\
      MSRA-NER      & NER   & 21K     & 2.3k     & 4.6K  & 7 & F1      \\
      XNLI          & NLI   & 392K    & 2.5K  & 2.5K  & 3 & Accuracy \\
      ChnSentiCorp  & SA    & 9.6K    & 1.2K  & 1.2K  & 2 & Accuracy \\
      LCQMC         & SS    & 240K    & 8.8K  & 12.5K & 2 & Accuracy \\
      BQ Corpus     & SS    & 100K    & 10K   & 10K   & 2  & Accuracy \\
      NLPCC-DBQA    & QA    & 182K    & 41K   & 82K   & 2 & mrr/F1   \\
        \hline \hline
		\end{tabular}
	\end{center}
    \caption{The details of Chinese NLP datasets. The \#Train, \#Dev and \#Test denote the size of the training set, development set and test set of corresponding corpus respectively. The \#label denotes the size of the label set of the corresponding corpus.}
	\label{chinese_data_detail}
\end{table*}

==> table_dataset_GLUE.tex <==
\begin{table*}[htb!]
    \tabcolsep 0.17in
	\begin{center}
	%\small
		\begin{tabular}{l|l|c|c|c|c|c}
		\hline \hline
			Corpus &Task& \#Train & \#Dev & \#Test   & \#Label &Metrics\\ \hline
			CoLA & Acceptability&8.5k & 1k & 1k & 2 & Matthews corr\\
			SST-2 & Sentiment&67k & 872 & 1.8k & 2 & Accuracy\\
			MNLI & NLI& 393k& 20k & 20k& 3 & Accuracy\\
            RTE & NLI &2.5k & 276 & 3k & 2 & Accuracy \\
            WNLI & NLI &634& 71& 146& 2 & Accuracy \\
			QQP & Paraphrase &364k & 40k & 391k& 2 & Accuracy/F1\\
            MRPC & Paraphrase &3.7k & 408 & 1.7k& 2&Accuracy/F1\\
			STS-B & Similarity &7k &1.5k& 1.4k &1 & Pearson/Spearman corr\\
			QNLI & QA/NLI& 108k &5.7k&5.7k&2& Accuracy\\
			AX & NLI & - & - & 1.1k & 3 & Matthews corr\\
		    \hline \hline
		\end{tabular}
	\end{center}
	\caption{The details of GLUE benchmark. The \#Train, \#Dev and \#Test denote the size of the training set, development set and test set of corresponding corpus respectively. The \#label denotes the size of the label set of the corresponding corpus. }
	    \label{glue_detail}
\end{table*} 

==> table_dataset_pretraining.tex <==
\begin{table}[htpb]
\tabcolsep 0.2in
  \centering
\small
\begin{center}
{
\begin{tabular}{@{}rcc@{}}
  \hline
  \hline
  Corpus Type     & English(\#tokens) & Chinese(\#tokens) \\ \hline
  Encyclopedia & 2021M & 7378M  \\ 
  BookCorpus  & 805M &  - \\ 
  News  & - &  1478M \\ \
  Dialog  & 4908M & 522M  \\ 
  IR Relevance Data & - & 4500M \\
  Discourse Relation Data & 171M & 1110M \\
\hline
\hline
\end{tabular}
} % small
\end{center}
\caption{The size of pre-training datasets. }
\label{training_dataset}
\end{table}

==> table_result_Chinese-Task.tex <==
\begin{table*}[htbp]
\tabcolsep 0.06in
  \centering
  \small
\begin{tabular}{c|c|cc|cc|cc|cc}
\hline \hline
\multirow{2}{*}{Task} & \multirow{2}{*}{Metrics} & \multicolumn{2}{c|}{BERT$_{BASE}$} & \multicolumn{2}{c|}{ERNIE 1.0$_{BASE}$} & \multicolumn{2}{c|}{ERNIE 2.0$_{BASE}$} & \multicolumn{2}{c}{ERNIE 2.0$_{LARGE}$} \\ \cline{3-10} 
                      &                          & Dev         & Test        & Dev               & Test             & Dev                 & Test               & Dev                 & Test                \\ \hline
CMRC 2018             & EM/F1                    & 66.3/85.9   & -           & 65.1/85.1         & -                & 69.1/88.6           & -                  & \textbf{71.5/89.9}  & -                   \\
DRCD                  & EM/F1                    & 85.7/91.6   & 84.9/90.9   & 84.6/90.9         & 84.0/90.5        & 88.5/93.8           & 88.0/93.4          & \textbf{89.7/94.7}  & \textbf{89.0/94.2}  \\
DuReader              & EM/F1                    & 59.5/73.1   & -           & 57.9/72.1         & -                & 61.3/74.9           & -                  & \textbf{64.2/77.3}  & -                   \\
MSRA-NER              & F1                       & 94.0        & 92.6        & 95.0              & 93.8             & 95.2                & 93.8               & \textbf{96.3}       & \textbf{95.0}       \\
XNLI                  & Accuracy                 & 78.1        & 77.2        & 79.9              & 78.4             & 81.2                & 79.7               & \textbf{82.6}       & \textbf{81.0}       \\
ChnSentiCorp          & Accuracy                 & 94.6        & 94.3       & 95.2              & 95.4             & 95.7                & 95.5               & \textbf{96.1}       & \textbf{95.8}       \\
LCQMC                 & Accuracy                 & 88.8        & 87.0        & 89.7              & 87.4             & \textbf{90.9}       & \textbf{87.9}      & \textbf{90.9}       & \textbf{87.9}       \\
BQ Corpus             & Accuracy                 & 85.9        & 84.8        & 86.1              & 84.8             & 86.4                & 85.0               & \textbf{86.5}       & \textbf{85.2}       \\
NLPCC-DBQA            & MRR/F1                   & 94.7/80.7   & 94.6/80.8   & 95.0/82.3         & 95.1/82.7        & 95.7/84.7           & 95.7/85.3          & \textbf{95.9/85.3}           & \textbf{95.8/85.8}           \\ \hline \hline

\end{tabular}
\caption{The results of 9 common Chinese NLP tasks. ERNIE 1.0 indicates our previous model ERNIE\cite{sun2019ernie}. The reported results are the average of five experimental results, and the state-of-the-art results are in bold.}
  \label{finetune_table}
\end{table*}

==> table_result_GLUE.tex <==
\begin{table*}[htbp]
\tabcolsep 0.06in
  \centering
  \small
\begin{tabular}{c|cc|ccc|cc}
\hline \hline
\multirow{3}{*}{Task(Metrics)}       & \multicolumn{2}{c|}{\textit{BASE model}}   & \multicolumn{5}{c}{\textit{LARGE model}}                                                                                                        \\ \cline{2-8} 
                                     & \multicolumn{2}{c|}{Test}                  & \multicolumn{3}{c|}{Dev}                                                              & \multicolumn{2}{c}{Test}                                 \\ \cline{2-8} 
                                     & BERT      & \multicolumn{1}{c|}{ERNIE 2.0} & \multicolumn{1}{c}{BERT} & \multicolumn{1}{c}{XLNet} & \multicolumn{1}{c|}{ERNIE 2.0} & \multicolumn{1}{c}{BERT} & \multicolumn{1}{c}{ERNIE 2.0} \\ \hline
CoLA (Matthew Corr.)                 & 52.1      & \textbf{55.2}                  & 60.6                     & 63.6                      & \textbf{65.4}                  & 60.5                     & \textbf{63.5}                 \\
SST-2 (Accuracy)                     & 93.5      & \textbf{95.0}                  & 93.2                     & 95.6                      & \textbf{96.0}                  & 94.9                     & \textbf{95.6}                 \\
MRPC (Accurary/F1)                   & 84.8/88.9 & \textbf{86.1/89.9}             & 88.0/-                   & 89.2/-                    & \textbf{89.7/-}                & 85.4/89.3                & \textbf{87.4/90.2}            \\
STS-B (Pearson Corr./Spearman Corr.) & 87.1/85.8 & \textbf{87.6/86.5}             & 90.0/-                   & 91.8/-                    & \textbf{92.3/-}                & 87.6/86.5                & \textbf{91.2/90.6}            \\
QQP (Accuracy/F1)                    & 89.2/71.2 & \textbf{89.8/73.2}             & 91.3/-                  & 91.8/-                    & \textbf{92.5/-}                & 89.3/72.1                & \textbf{90.1/73.8}            \\
MNLI-m/mm (Accuracy)                    & 84.6/83.4      & \textbf{86.1/85.5}                  & 86.6/-                     & \textbf{89.8/-}                      & 89.1/-                  & 86.7/85.9                     & \textbf{88.7/88.8}                 \\
QNLI (Accuracy)                    & 90.5      & \textbf{92.9}                  & 92.3                     & 93.9                      & \textbf{94.3}                  & 92.7                     & \textbf{94.6}                 \\
RTE (Accuracy)                       & 66.4      & \textbf{74.8}                  & 70.4                     & 83.8                      & \textbf{85.2}                  & 70.1                     & \textbf{80.2}                 \\
WNLI (Accuracy)                      & \textbf{65.1}      & \textbf{65.1}                  & -                        & -                         & -                              & 65.1                     & \textbf{67.8}                 \\ 
AX(Matthew Corr.)           & 34.2  & \textbf{37.4}  &   - & - & -  & 39.6 & \textbf{48.0}    \\    \hline         
Score                                & 78.3      & \textbf{80.6}                  & -                        & -                         & -                              & 80.5                     & \textbf{83.6}                 \\ \hline \hline
\end{tabular}
\caption{The results on GLUE benchmark, where the results on dev set are the median of five experimental results and the results on test set are scored by the GLUE evaluation server (\url{https://gluebenchmark.com/leaderboard}). The state-of-the-art results are in bold. All of the fine-tuned models of AX is trained by the data of MNLI.}
\label{glue_test}
\end{table*}

==> table_setting_Chinese-Task.tex <==
\begin{table}[htbp]
\tabcolsep 0.08in
\small
\begin{center}

{
\begin{tabular}{@{}c|ccc|ccc@{}}
  \hline \hline
   \multirow{2}{*}{Task}      &  \multicolumn{3}{c|}{\textit{BASE}} & \multicolumn{3}{c}{\textit{LARGE}} \\ \cline{2-7}
                &  Epoch & Learning Rate & Batch Size &  Epoch & Learning Rate & Batch Size\\ \hline 
  CMRC 2018  & 2 & 3e-5 & 64 & 2 & 3e-5 & 64 \\
  DRCD  & 2 & 5e-5 & 64 & 2 & 3e-5 & 64 \\
  DuReader  & 2 & 5e-5 & 64 & 2 & 2e-5 & 64 \\
  MSRA-NER  & 6 & 5e-5 & 16    & 6 & 1e-5 & 16 \\
  XNLI  & 3 & 1e-4 & 65536(\#tokens) & 3 & 4e-5 & 65536(\#tokens) \\
  ChnSentiCorp  & 10 & 5e-5 & 24  & 10 & 1e-5 & 24  \\
  LCQMC  & 3 & 2e-5 & 32  & 3 & 5e-6 & 32  \\
  BQ Corpus  & 3 & 3e-5 & 64  & 3 & 1.5e-5 & 64  \\
  NLPCC-DBQA  & 3 & 2e-5 & 64 & 3 & 1e-5 & 64 \\
\hline \hline
\end{tabular}
} % small
\end{center}
\caption{The Experiment Settings for Chinese datasets}
\label{chinese_finetune_setting}
\end{table}

==> table_setting_GLUE.tex <==
\begin{table}[htbp]
\tabcolsep 0.11in
\small
\begin{center}

{
\begin{tabular}{@{}c|ccc|ccc@{}}
  \hline \hline 
   \multirow{2}{*}{Task}      &  \multicolumn{3}{c|}{\textit{BASE}} & \multicolumn{3}{c}{\textit{LARGE}} \\ \cline{2-7}
                &  Epoch & Learning Rate & Batch Size &  Epoch & Learning Rate & Batch Size\\ \hline 
  CoLA  & 3 & 3e-5 & 64  & 5 & 3e-5 & 32 \\
  SST-2  & 4 & 2e-5 & 256 & 4 & 2e-5 & 64  \\
  MRPC  & 4 & 3e-5 & 32 & 4 & 3e-5 & 16 \\
  STS-B  & 3 & 5e-5 & 128 & 3 & 5e-5 & 128 \\
  QQP  & 3 & 3e-5 & 256  & 3 & 5e-5 & 256  \\
  MNLI  & 3 & 3e-5 & 512 & 3 & 3e-5 & 256 \\
  QNLI  & 4 & 2e-5 & 256 & 4 & 2e-5 & 256  \\
  RTE  & 4 & 2e-5 & 4 & 5 & 3e-5 & 16  \\
  WNLI  & 4 & 2e-5 & 8 & 4 & 2e-5 & 8   \\
\hline \hline
\end{tabular}
} % small
\end{center}
\caption{The Experiment settings for GLUE dataset}
\label{GLUE_finetune_setting}
\end{table}
